International Workshop on Next Generation Gamma-Ray Source

A workshop on The Next Generation Gamma-Ray Sources sponsored by the Office of Nuclear Physics at the Department of Energy, was held November 17--19, 2016 in Bethesda, Maryland. The goals of the workshop were to identify basic and applied research opportunities at the frontiers of nuclear physics that would be made possible by the beam capabilities of an advanced laser Compton beam facility. To anchor the scientific vision to realistically achievable beam specifications using proven technologies, the workshop brought together experts in the fields of electron accelerators, lasers, and optics to examine the technical options for achieving the beam specifications required by the most compelling parts of the proposed research programs. An international assembly of participants included current and prospective $\gamma$-ray beam users, accelerator and light-source physicists, and federal agency program managers. Sessions were organized to foster interactions between the beam users and facility developers, allowing for information sharing and mutual feedback between the two groups. The workshop findings and recommendations are summarized in this whitepaper.

==> bibliography.tex <==
%%%%%%%%%%% Bibliography %%%%%%%%%%%%%%%%
\begin{thebibliography}{}
	
%% new items from Nuclear Structure
\bibitem{Bec17}T.~Beck {\it et al.}, Phys.\ Rev.\ Lett.\ {\bf 118}, 212502 (2017).

\bibitem{rein10} P.-G. Reinhard and W. ~Nazarewicz, Phys. Rev. C {\bf 81}, 051303, (2010) 
	
%\bibitem[{\citenamefont{Piekarewicz}(2011)}]{piek11}
%\bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Piekarewicz}},
%  \bibinfo{journal}{Phys. Rev. C} \textbf{\bibinfo{volume}{83}},
%  \bibinfo{pages}{034319} (\bibinfo{year}{2011}).
%
%\bibitem[{\citenamefont{Tamii et~al.}(2011)\citenamefont{Tamii, Poltoratska,
%  von Neumann-Cosel, Fujita, Adachi, Bertulani, Carter, Dozono, Fujita, Fujita
%  et~al.}}]{tami11}
%\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Tamii}},
%  \bibinfo{author}{\bibfnamefont{I.}~\bibnamefont{Poltoratska}},
%  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{von Neumann-Cosel}},
%  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Fujita}},
%  \bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Adachi}},
%  \bibinfo{author}{\bibfnamefont{C.~A.} \bibnamefont{Bertulani}},
%  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Carter}},
%  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Dozono}},
%  \bibinfo{author}{\bibfnamefont{H.}~\bibnamefont{Fujita}},
%  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Fujita}},
%  \bibnamefont{et~al.}, \bibinfo{journal}{Phys. Rev. Lett.}
%  \textbf{\bibinfo{volume}{107}}, \bibinfo{pages}{062502}
%  (\bibinfo{year}{2011}).
%
%\bibitem[{\citenamefont{Rossi et~al.}(2013)\citenamefont{Rossi, Adrich, Aksouh,
%  Alvarez-Pol, Aumann, Benlliure, B\"ohmer, Boretzky, Casarejos, Chartier
%  et~al.}}]{ross13}
%\bibinfo{author}{\bibfnamefont{D.~M.} \bibnamefont{Rossi}},
%  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Adrich}},
%  \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Aksouh}},
%  \bibinfo{author}{\bibfnamefont{H.}~\bibnamefont{Alvarez-Pol}},
%  \bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Aumann}},
%  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Benlliure}},
%  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{B\"ohmer}},
%  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Boretzky}},
%  \bibinfo{author}{\bibfnamefont{E.}~\bibnamefont{Casarejos}},
%  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Chartier}},
%  \bibnamefont{et~al.}, \bibinfo{journal}{Phys. Rev. Lett.}
%  \textbf{\bibinfo{volume}{111}}, \bibinfo{pages}{242503}
%  (\bibinfo{year}{2013}).
%
%\bibitem[{\citenamefont{Roca-Maza et~al.}({2015})\citenamefont{Roca-Maza,
%  Vinas, Centelles, Agrawal, Colo, Paar, Piekarewicz, and Vretenar}}]{roca15}
%\bibinfo{author}{\bibfnamefont{X.}~\bibnamefont{Roca-Maza}},
%  \bibinfo{author}{\bibfnamefont{X.}~\bibnamefont{Vinas}},
%  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Centelles}},
%  \bibinfo{author}{\bibfnamefont{B.~K.} \bibnamefont{Agrawal}},
%  \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Colo}},
%  \bibinfo{author}{\bibfnamefont{N.}~\bibnamefont{Paar}},
%  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Piekarewicz}},
%  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Vretenar}},
%  \bibinfo{journal}{Phys. Rev. C} \textbf{\bibinfo{volume}{{92}}},
%  \bibinfo{pages}{{064304}} (\bibinfo{year}{{2015}}).
%
%\bibitem[{\citenamefont{Baldo and Burgio}(2016)}]{bald16}
%\bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Baldo}} \bibnamefont{and}
%  \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Burgio}},
%  \bibinfo{journal}{Prog. Part. Nucl. Phys.} \textbf{\bibinfo{volume}{91}},
%  \bibinfo{pages}{203} (\bibinfo{year}{2016}).
%
%\bibitem[{\citenamefont{Goriely et~al.}(2004)\citenamefont{Goriely, Khan, and
%  Samyn}}]{gori04}
%\bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Goriely}},
%  \bibinfo{author}{\bibfnamefont{E.}~\bibnamefont{Khan}}, \bibnamefont{and}
%  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Samyn}},
%  \bibinfo{journal}{Nucl. Phys.} \textbf{\bibinfo{volume}{A739}},
%  \bibinfo{pages}{331} (\bibinfo{year}{2004}).
%
%\bibitem[{\citenamefont{Litvinova et~al.}(2009)\citenamefont{Litvinova, Ring,
%  Tselyaev, and Langanke}}]{litv09}
%\bibinfo{author}{\bibfnamefont{E.}~\bibnamefont{Litvinova}},
%  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Ring}},
%  \bibinfo{author}{\bibfnamefont{V.}~\bibnamefont{Tselyaev}}, \bibnamefont{and}
%  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Langanke}},
%  \bibinfo{journal}{Phys. Rev. C} \textbf{\bibinfo{volume}{79}},
%  \bibinfo{pages}{054312} (\bibinfo{year}{2009}).
%
%\bibitem[{\citenamefont{Daoutidis and Goriely}(2012)}]{daou12}
%\bibinfo{author}{\bibfnamefont{I.}~\bibnamefont{Daoutidis}} \bibnamefont{and}
%  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Goriely}},
%  \bibinfo{journal}{Phys. Rev. C} \textbf{\bibinfo{volume}{86}},
%  \bibinfo{pages}{034328} (\bibinfo{year}{2012}).
%
%\bibitem[{\citenamefont{Tonchev et~al.}(2017)\citenamefont{Tonchev, Tsoneva,
%  Bhatia, Arnold, Goriely, Hammond, Kelley, Kwan, Lenske, Piekarewicz
%  et~al.}}]{tonc17}
%\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Tonchev}},
%  \bibinfo{author}{\bibfnamefont{N.}~\bibnamefont{Tsoneva}},
%  \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Bhatia}},
%  \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Arnold}},
%  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Goriely}},
%  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Hammond}},
%  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Kelley}},
%  \bibinfo{author}{\bibfnamefont{E.}~\bibnamefont{Kwan}},
%  \bibinfo{author}{\bibfnamefont{H.}~\bibnamefont{Lenske}},
%  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Piekarewicz}},
%  \bibnamefont{et~al.}, \bibinfo{journal}{Phys. Lett. B}
%  \textbf{\bibinfo{volume}{773}}, \bibinfo{pages}{20} (\bibinfo{year}{2017}).
%
%\bibitem[{\citenamefont{Savran et~al.}(2006{\natexlab{a}})\citenamefont{Savran,
%  Babilon, van~den Berg, Harakeh, Hasper, Matic, W\"ortche, and
%  Zilges}}]{savr06}
%\bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Savran}},
%  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Babilon}},
%  \bibinfo{author}{\bibfnamefont{A.~M.} \bibnamefont{van~den Berg}},
%  \bibinfo{author}{\bibfnamefont{M.~N.} \bibnamefont{Harakeh}},
%  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Hasper}},
%  \bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Matic}},
%  \bibinfo{author}{\bibfnamefont{H.~J.} \bibnamefont{W\"ortche}},
%  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Zilges}},
%  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{97}},
%  \bibinfo{pages}{172502} (\bibinfo{year}{2006}{\natexlab{a}}).
%
% \bibitem{Sav18}D.~Savran {\it et al.}, Phys.\ Lett.\ {\bf B786}, 16 (2018).
%
%\bibitem[{\citenamefont{Krumbholz et~al.}(2015)\citenamefont{Krumbholz, von
%  Neumann-Cosel, Hashimoto, Tamii, Adachi, Bertulani, Fujita, Fujita, Ganioglu,
%  Hatanaka et~al.}}]{krum15}
%\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Krumbholz}},
%  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{von Neumann-Cosel}},
%  \bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Hashimoto}},
%  \bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Tamii}},
%  \bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Adachi}},
%  \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Bertulani}},
%  \bibinfo{author}{\bibfnamefont{H.}~\bibnamefont{Fujita}},
%  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Fujita}},
%  \bibinfo{author}{\bibfnamefont{E.}~\bibnamefont{Ganioglu}},
%  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Hatanaka}},
%  \bibnamefont{et~al.}, \bibinfo{journal}{Phys. Lett. B}
%  \textbf{\bibinfo{volume}{744}}, \bibinfo{pages}{7} (\bibinfo{year}{2015}).
%
%  \bibitem{Isa18}J.~Isaak {\it et al.}, Phys.\ Lett., in press.
	
	
%% End new items

%% New Items from QCD folks

\bibitem{Hagelstein:2015egb}
F.~Hagelstein, R.~Miskimen and V.~Pascalutsa,
%``Nucleon Polarizabilities: from Compton Scattering to Hydrogen Atom,''
Prog.\ Part.\ Nucl.\ Phys.\  {\bf 88} (2016) 29
doi:10.1016/j.ppnp.2015.12.001
[arXiv:1512.03765 [nucl-th]].
%%CITATION = doi:10.1016/j.ppnp.2015.12.001;%%
%35 citations counted in INSPIRE as of 05 Nov 2018

\bibitem{Wissmann:2004}
F. Wissmann, {\it Compton Scattering: Investigating the Structure of the Nucleon with Real Photons}, Springer Tracts in Modern Physics, Volume 200 (2004).

\bibitem{Pasquini:2018wbl} 
B.~Pasquini and M.~Vanderhaeghen,
%``Dispersion Theory in Electromagnetic Interactions,''
Ann.\ Rev.\ Nucl.\ Part.\ Sci.\  {\bf 68}, 75 (2018)
doi:10.1146/annurev-nucl-101917-020843
[arXiv:1805.10482 [hep-ph]].
%%CITATION = doi:10.1146/annurev-nucl-101917-020843;%%
%1 citations counted in INSPIRE as of 16 Nov 2018

%\cite{Gasser:2015dwa}
\bibitem{Gasser:2015dwa} 
J.~Gasser, M.~Hoferichter, H.~Leutwyler and A.~Rusetsky,
%``Cottingham formula and nucleon polarisabilities,''
Eur.\ Phys.\ J.\ C {\bf 75} (2015) 375
[arXiv:1506.06747 [hep-ph]].
%%CITATION = ARXIV:1506.06747;%%
%4 citations counted in INSPIRE as of 22 Oct 2015

%\cite{higherorderpols}
\bibitem{higherorderpols} J.~A.~McGovern, D.~R.~Phillips and
H.~W.~Grie{\ss}hammer, % : \emph{Compton Scattering from the Proton in an
% Effective Field Theory with Explicit Delta Degrees of Freedom},
Eur.\ Phys.\ J.\ A  \textbf{49} (2013) 12 [arXiv:1210.4104 [nucl-th]].

%\cite{Lvov:1993fp}
\bibitem{WalkerLoud:2012bg}
A.~Walker-Loud, C.~E.~Carlson and G.~A.~Miller,
%  ``The Electromagnetic Self-Energy Contribution to $M_p - M_n$ and the Isovector
%  Nucleon Magnetic Polarizability,''
Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 232301 
[arXiv:1203.0254 [nucl-th]].
%%CITATION = ARXIV:1203.0254;%%

%\cite{Birse:2012eb}
\bibitem{Birse:2012eb}
M.~C.~Birse and J.~A.~McGovern,
%``Proton polarisability contribution to the Lamb shift in muonic hydrogen at fourth order in chiral perturbation theory,''
Eur.\ Phys.\ J.\ A {\bf 48} (2012) 120
doi:10.1140/epja/i2012-12120-8
[arXiv:1206.3030 [hep-ph]].
%%CITATION = doi:10.1140/epja/i2012-12120-8;%%
%96 citations counted in INSPIRE as of 05 Nov 2018

%\cite{Pohl:2013yb}
\bibitem{Pohl:2013yb} 
R.~Pohl, R.~Gilman, G.~A.~Miller and K.~Pachucki,
%  ``Muonic hydrogen and the proton radius puzzle,''
Ann.\ Rev.\ Nucl.\ Part.\ Sci.\  {\bf 63} (2013) 175
[arXiv:1301.0905 [physics.atom-ph]].
%%CITATION = ARXIV:1301.0905;%%
%75 citations counted in INSPIRE as of 18 juin 2015


%\cite{NAS}
\bibitem{NAS} Committee on the Assessment of and Outlook for Nuclear Physics,
National Research Council of the National Academies, ``Nuclear Physics:
Exploring the Heart of Matter'', 2012%,
%  \href{http://sites.nationalacademies.org/bpa/BPA_055628}
%  {sites.nationalacademies.org/bpa/BPA$\_$055628}
.

%\cite{nupecc2017}
\bibitem{nupecc2017} European Science Foundation, ``NuPECC Long Range Plan
2017 -- Perspectives in Nuclear Physics'', 2017%,
%  \href{http://www.nupecc.org}{www.nupecc.org}
.

%\cite{Lujan:2014qga}
\bibitem{Lujan:2014qga} 
M.~Lujan, A.~Alexandru, W.~Freeman and F.~Lee,
%``Finite volume study of electric polarizabilities from lattice QCD,''
PoS LATTICE {\bf 2014} (2014) 153
[arXiv:1411.0047 [hep-lat]].
%%CITATION = ARXIV:1411.0047;%%
%3 citations counted in INSPIRE as of 30 May 2015

%\cite{Engelhardt:2011qq}
\bibitem{Engelhardt:2011qq} 
M.~Engelhardt,
%``Exploration of the electric spin polarizability of the neutron in lattice QCD,''
PoS LATTICE {\bf 2011} (2011) 153
[arXiv:1111.3686 [hep-lat]].
%%CITATION = ARXIV:1111.3686;%%
%6 citations counted in INSPIRE as of 30 May 2015

%\cite{Beane:2015yha}
\bibitem{Beane:2015yha}
S.~R.~Beane {\it et al.} [NPLQCD Collaboration],
%``Ab initio Calculation of the np→dγ Radiative Capture Process,''
Phys.\ Rev.\ Lett.\  {\bf 115} (2015) no.13,  132001
doi:10.1103/PhysRevLett.115.132001
[arXiv:1505.02422 [hep-lat]].
%%CITATION = doi:10.1103/PhysRevLett.115.132001;%%
%40 citations counted in INSPIRE as of 05 Nov 2018

%\cite{Detmold:2015daa}
\bibitem{Detmold:2015daa} 
W.~Detmold, K.~Orginos, A.~Parreno, M.~J.~Savage, B.~C.~Tiburzi, S.~R.~Beane and E.~Chang,
%``Unitary Limit of Two-Nucleon Interactions in Strong Magnetic Fields,''
Phys.\ Rev.\ Lett.\  {\bf 116}, no. 11, 112301 (2016)
doi:10.1103/PhysRevLett.116.112301
[arXiv:1508.05884 [hep-lat]].
%%CITATION = doi:10.1103/PhysRevLett.116.112301;%%
%17 citations counted in INSPIRE as of 05 Nov 2018

%\cite{Lujan:2014kia}
\bibitem{Lujan:2014kia}
M.~Lujan, A.~Alexandru, W.~Freeman and F.~Lee,
%``Electric polarizability of neutral hadrons from dynamical lattice QCD ensembles,''
Phys.\ Rev.\ D {\bf 89} (2014) no.7,  074506
doi:10.1103/PhysRevD.89.074506
[arXiv:1402.3025 [hep-lat]].
%%CITATION = doi:10.1103/PhysRevD.89.074506;%%
%19 citations counted in INSPIRE as of 05 Nov 2018

%\cite{Griesshammer:2015ahu}
\bibitem{Griesshammer:2015ahu} 
H.~W.~Griesshammer, J.~A.~McGovern and D.~R.~Phillips,
%``Nucleon Polarisabilities at and Beyond Physical Pion Masses,''
Eur.\ Phys.\ J.\ A {\bf 52}, no. 5, 139 (2016)
doi:10.1140/epja/i2016-16139-5
[arXiv:1511.01952 [nucl-th]].
%%CITATION = doi:10.1140/epja/i2016-16139-5;%%
%13 citations counted in INSPIRE as of 05 Nov 2018

%\cite{Olmos:2001}
\bibitem{Olmos:2001} V.~Olmos de Le\'on et al., Eur.\ Phys.\ J.\ {\bf A10 }
(2001) 207. 

%\cite{Levchuk:1999zy}
\bibitem{Levchuk:1999zy} M.~I.~Levchuk and A.~I.~L'vov,
% ``Deuteron Compton scattering below pion photoproduction threshold,''
Nucl.\ Phys.\ A {\bf 674} (2000) 449 [nucl-th/9909066].
%% CITATION = NUCL-TH/9909066;%%
% 45 citations counted in INSPIRE as of 24 Apr 2015

%\cite{Gryniuk:2015eza}
\bibitem{Gryniuk:2015eza} 
O.~Gryniuk, F.~Hagelstein and V.~Pascalutsa,
%``Evaluation of the forward Compton scattering off protons: Spin-independent amplitude,''
Phys.\ Rev.\ D {\bf 92} (2015) 074031
%  doi:10.1103/PhysRevD.92.074031
[arXiv:1508.07952 [nucl-th]].
%%CITATION = doi:10.1103/PhysRevD.92.074031;%%
%4 citations counted in INSPIRE as of 14 Sep 2017

%\cite{Pasquini:2017ehj}
\bibitem{Pasquini:2017ehj} 
B.~Pasquini, P.~Pedroni and S.~Sconfietti,
%``First extraction of the scalar proton dynamical polarizabilities from real Compton scattering data,''
Phys.\ Rev.\ C {\bf 98}, no. 1, 015204 (2018)
doi:10.1103/PhysRevC.98.015204
[arXiv:1711.07401 [hep-ph]].
%%CITATION = doi:10.1103/PhysRevC.98.015204;%%
%3 citations counted in INSPIRE as of 05 Nov 2018

%\cite{Krupina:2017pgr}
\bibitem{Krupina:2017pgr} 
N.~Krupina, V.~Lensky and V.~Pascalutsa,
%``Partial-wave analysis of proton Compton scattering data below the pion-production threshold,''
Phys.\ Lett.\ B {\bf 782}, 34 (2018)
doi:10.1016/j.physletb.2018.04.066
[arXiv:1712.05349 [nucl-th]].
%%CITATION = doi:10.1016/j.physletb.2018.04.066;%%
%4 citations counted in INSPIRE as of 05 Nov 2018


%\cite{Griesshammer:2013vga}
\bibitem{Griesshammer:2013vga} H.~W.~Grie{\ss}hammer,
% ``Dissecting Deuteron Compton Scattering I: The Observables with Polarised
% Initial States,''
Eur.\ Phys.\ J.\ A {\bf 49} (2013) 100; Erratua: Eur.\ Phys.\ J.\ A {\bf 53}
(2017) 113 and  Eur.\ Phys.\ J.\ A {\bf 54} (2018) 57
[arXiv:1304.6594 [nucl-th]].
%% CITATION = doi:10.1140/epja/i2013-13100-2;%%
% 5 citations counted in INSPIRE as of 10 May 2017

%\cite{Sokhoyan:2016yrc}
\bibitem{Sokhoyan:2016yrc} 
V.~Sokhoyan {\it et al.} [A2 Collaboration],
%``Determination of the scalar polarizabilities of the proton using beam asymmetry $\Sigma_{3}$ in Compton scattering,''
Eur.\ Phys.\ J.\ A {\bf 53}, no. 1 (2017) 14 
%doi:10.1140/epja/i2017-12203-0
[arXiv:1611.03769 [nucl-ex]].
%%CITATION = doi:10.1140/epja/i2017-12203-0;%%
%1 citations counted in INSPIRE as of 14 Sep 2017

%\cite{Martel:2017pln}
\bibitem{Martel:2017pln} 
P.~Martel {\it et al.} [A2 Collaboration],
%``Compton Scattering Program Studying Nucleon Polarizabilities,''
EPJ Web Conf.\  {\bf 142} (2017) 01021.
%  doi:10.1051/epjconf/201714201021
%%CITATION = doi:10.1051/epjconf/201714201021;%%

%\cite{Collicott:2015}
\bibitem{Collicott:2015} C.~Collicott, {\it PhD Thesis}, Dalhousie University
(2015) % \url{https://wwwa2.kph.uni-mainz.de/images/publications/phd/thesis_Collicott-Cristina-2015.pdf}


\bibitem{Lensky:2015awa} 
V.~Lensky, J.~McGovern and V.~Pascalutsa,
%``Predictions of covariant chiral perturbation theory for nucleon polarisabilities and polarised Compton scattering,''
Eur.\ Phys.\ J.\ C {\bf 75}, no. 12, 604 (2015)
doi:10.1140/epjc/s10052-015-3791-0
[arXiv:1510.02794 [hep-ph]].
%%CITATION = doi:10.1140/epjc/s10052-015-3791-0;%%
%21 citations counted in INSPIRE as of 19 Nov 2018

%\cite{Griesshammer:2017txw}
\bibitem{Griesshammer:2017txw} H.~W.~Grie{\ss}hammer, J.~A.~McGovern and
D.~R.~Phillips,
% ``Comprehensive Study of Observables in Compton Scattering on the
% Nucleon,''
Eur.\ Phys.\ J.\ A {\bf 54} (2018) 37
[arXiv:1711.11546 [nucl-th]]. 
%% CITATION = ARXIV:1711.11546;%%

%\cite{Margaryan:2018opu}
\bibitem{Margaryan:2018opu} 
A.~Margaryan, B.~Strandberg, H.~W.~Griesshammer, J.~A.~Mcgovern, D.~R.~Phillips and D.~Shukla,
%``Elastic Compton scattering from$^{3}$He and the role of the Delta,''
Eur.\ Phys.\ J.\ A {\bf 54}, no. 7, 125 (2018)
doi:10.1140/epja/i2018-12554-x
[arXiv:1804.00956 [nucl-th]].
%%CITATION = doi:10.1140/epja/i2018-12554-x;%%
%1 citations counted in INSPIRE as of 05 Nov 2018

%\cite{Babusci:1998ww}
\bibitem{Babusci:1998ww}
D.~Babusci, G.~Giordano, A.~I.~L'vov, G.~Matone and A.~M.~Nathan,
%``Low-energy Compton scattering of polarized photons on polarized nucleons,''
Phys.\ Rev.\ C {\bf 58} (1998) 1013
[hep-ph/9803347] .
%%CITATION = HEP-PH/9803347;%%
%95 citations counted in INSPIRE as of 12 Feb 2014

%\cite{Hildebrandt:2003md}
\bibitem{Hildebrandt:2003md} R.~P.~Hildebrandt, H.~W.~Grie{\ss}hammer and T.~R.~Hemmert,
%``Spin polarisabilities of the nucleon from polarised low-energy Compton scattering,''
Eur.\ Phys.\ J.\ A {\bf 20} (2004) 329
[arXiv:nucl-th/0308054].

%\cite{Holstein:1999uu}
%\bibitem{Holstein:1999uu}
%  B.~R.~Holstein, D.~Drechsel, B.~Pasquini and M.~Vanderhaeghen,
%  %``Higher order polarizabilities of the proton,''
%  Phys.\ Rev.\  C {\bf 61} (2000) 034316
%  [arXiv:hep-ph/9910427].
%  %%CITATION = PHRVA,C61,034316;%%

%\cite{Hildebrandt:2003fm}
\bibitem{Hildebrandt:2003fm} 
R.~P.~Hildebrandt, H.~W.~Grie{\ss}hammer, T.~R.~Hemmert and B.~Pasquini,
%``Signatures of chiral dynamics in low-energy compton scattering off the nucleon,''
Eur.\ Phys.\ J.\ A {\bf 20} (2004) 293
%doi:10.1140/epja/i2003-10144-9
[nucl-th/0307070].
%%CITATION = doi:10.1140/epja/i2003-10144-9;%%
%84 citations counted in INSPIRE as of 13 Sep 2017


%\cite{Pasquini:2007hf}
\bibitem{Pasquini:2007hf} 
B.~Pasquini, D.~Drechsel and M.~Vanderhaeghen,
%``Proton spin polarizabilities from polarized Compton scattering,''
Phys.\ Rev.\ C {\bf 76}, 015203 (2007)
doi:10.1103/PhysRevC.76.015203
[arXiv:0705.0282 [hep-ph]].
%%CITATION = doi:10.1103/PhysRevC.76.015203;%%
%39 citations counted in INSPIRE as of 06 Nov 2018

\bibitem{Drechsel:1999rf} 
D.~Drechsel, M.~Gorchtein, B.~Pasquini and M.~Vanderhaeghen,
%``Fixed t subtracted dispersion relations for Compton Scattering off the nucleon,''
Phys.\ Rev.\ C {\bf 61}, 015204 (1999)
doi:10.1103/PhysRevC.61.015204
[hep-ph/9904290].
%%CITATION = doi:10.1103/PhysRevC.61.015204;%%
%96 citations counted in INSPIRE as of 16 Nov 2018

%\cite{Myers:2015aba}
\bibitem{Myers:2015aba} 
L.~S.~Myers {\it et al.},
%``Compton Scattering from the Deuteron below Pion-Production Threshold,''
Phys.\ Rev.\ C {\bf 92}, no. 2, 025203 (2015)
doi:10.1103/PhysRevC.92.025203
[arXiv:1503.08094 [nucl-ex]].
%%CITATION = doi:10.1103/PhysRevC.92.025203;%%
%13 citations counted in INSPIRE as of 06 Nov 2018


\bibitem{Sikora:2017rfk} 
M.~H.~Sikora {\it et al.},
%``Compton scattering from $^4$He at 61 MeV,''
Phys.\ Rev.\ C {\bf 96}, no. 5, 055209 (2017).
doi:10.1103/PhysRevC.96.055209
%%CITATION = doi:10.1103/PhysRevC.96.055209;%%


\bibitem{3HeHIGS} G.~Feldman et al., proposal for HIGS experiment E-08-16: Compton Scattering from 3He.  


\bibitem{Kossert:2002jc} 
K.~Kossert {\it et al.},
%``Neutron polarizabilities investigated by quasifree Compton scattering from the deuteron,''
Phys.\ Rev.\ Lett.\  {\bf 88}, 162301 (2002)
doi:10.1103/PhysRevLett.88.162301
[nucl-ex/0201015].
%%CITATION = doi:10.1103/PhysRevLett.88.162301;%%
%39 citations counted in INSPIRE as of 08 Nov 2018

\bibitem{Kossert:2002ws} 
K.~Kossert {\it et al.},
%``Quasifree Compton scattering and the polarizabilities of the neutron,''
Eur.\ Phys.\ J.\ A {\bf 16}, 259 (2003)
doi:10.1140/epja/i2002-10093-9
[nucl-ex/0210020].
%%CITATION = doi:10.1140/epja/i2002-10093-9;%%
%47 citations counted in INSPIRE as of 08 Nov 2018

%% --------------------	
	\bibitem{Bec01} D.~H.~Beck and B.~Holstein, Int. J. Mod. Phys. E {\bf 10}, 1 (2001).
	
	\bibitem{Beck01} D.~H.~Beck and R.~D.~McKeown, Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf 51}, 189 (2001).
	
	\bibitem{Beck03} D.~H.~Beck, Prog.\ Nucl.\ Part.\ Phys.\ {\bf 50}, 429 (2003).
	
	\bibitem{Beise05} E.~J.~Beise, M.~L.~Pitt, and D.~T.~Spayde, Prog.\ Nucl.\ Part.\ Phys.\ {\bf 54}, 289 (2005).
	
	\bibitem{Ade85} E.~G.~Adelberger and W.~C.~Haxton, Ann. Rev. Nucl. Part. Sci. {\bf 35}, 501 (1985).
	
	\bibitem{Bow1} J.~D.~Bowman, G.~T.~Garvey, and M.~B.~Johnson, Ann.\ Rev.\ 
	Nucl.\ Part.\ Sci.\ {\bf 43}, 829 (1993).
	
	\bibitem{Tom} S.~Tomsovic, M.~B.~Johnson, A.~Hayes, and J.~D.~Bowman, 
	Phys.\ Rev.\ C {\bf 62}, 054607 (2000).
	
	\bibitem{Woo97} C.~S.~Wood {\it et al.}, Science {\bf 275}, 1759 (1997).
	
	\bibitem{Zel57} Y.~B.~Zeldovich, Sov.\ Phys.\ JETP {\bf 6}, 1184 (1957).
	
	\bibitem{Fla80} V.~V.~Flambaum and I.~B.~Khriplovich, Sov.\ Phys.\ JETP {\bf 52}, 835 (1980).
	
	\bibitem{Tsi09}K.~Tsigutkin {\it et al.}, Phys.\ Rev.\ Lett.\ {\bf 103}, 071601 (2009).
	
	\bibitem{Pre03} G. Prezeau, M. Ramsey-Musolf, and P. Vogel, Phys. Rev. D {\bf 68}, 034016 (2003).
	
	\bibitem{Bowman2014} J. D. Bowman and V. Gudkov, Phys. Rev. C {\bf 90}, 065503 (2014).
	
	\bibitem{Wasem12} J. Wasem, Phys. Rev. C {\bf 85}, 022501(R) (2012). 
	
	\bibitem{KITP} Frontiers in Nuclear Physics, KITP workshop, Aug. 22 to Nov. 4, 2016.
	
	\bibitem{Dan} G. S. Danilov, Phys. Lett. {\bf 18}, 40 (1965).

	\bibitem{Zhu05} S. L. Zhu {\it et al.}, Nucl. Phys. A {\bf 748}, 435 (2005).
	\bibitem{Girlanda:2008ts} L.~Girlanda,
	%``On a redundancy in the parity-violating 2-nucleon contact Lagrangian,''
	Phys.\ Rev.\ C {\bf 77}, 067001 (2008)
	[arXiv:0804.0772 [nucl-th]].
	%%CITATION = ARXIV:0804.0772;%%
	
	\bibitem{Phillips:2014kna} 
	D.~R.~Phillips, D.~Samart, and C.~Schat,
	Phys.\ Rev.\ Lett.\ {\bf 114}, 062301 (2015).
	
	\bibitem{Schindler2016} M. R. Schindler, R. P. Springer, and J. Vanasse, Phys. Rev. C {\bf 93}, 025502 (2016).
	
	\bibitem{Snow2015} W. M. Snow {\it et al.}, Rev. Sci. Instrum. {\bf 86}, 055101 (2015).
	
	\bibitem{INCITE} A.~Walker-Loud, E.~Berkowitz, W.~Haxton, T.~Kurth,  A.~Nicholson, and J.~Wasem, 2016 Incite Award, {\it First Lattice QCD Calculation of the $I=2$ Two-Nucleon Parity Violating Amplitude}. 
	
	\bibitem{Kurth:2015cvl} 
	T.~Kurth {\it et al.}, %E.~Berkowitz, E.~Rinaldi, P.~Vranas, A.~Nicholson, M.~Strother, A.~Walker-Loud, and E.~Rinaldi,
	%``Nuclear Parity Violation from Lattice QCD,''
	PoS LATTICE {\bf 2015}, 329 (2016).
	
	\bibitem{Earle88} E.~D.~Earle {\it et al.}, %A.~B.~McDonald, S.~H.~Kinder, E.~T.~H.~Clifford, J.~J.~Hill, G.~H.~Keech, T.~E.~Chupp, and M.~B.~Schneider, 
	Can.~J.~Phys. {\bf 66}, 534 (1988).
	
	\bibitem{Knyaz'kov:1984zz} 
	V.~A.~Knyaz'kov {\it et al.}, %E.~A.~Kolomenskii, V.~M.~Lobashov, V.~A.~Nazarenko, A.~N.~Pirozhkov, A.~I.~Shablii, E.~V.~Shul'gina and Y.~V.~Sobolev,
	%``A new experimental study of the circular polarization of np capture gamma-rays,''
	Nucl.\ Phys.\ A {\bf 417}, 209 (1984).
	%%CITATION = NUPHA,A417,209;%%
	
	\bibitem{Sinclair00} C. Sinclair {\it et al.}, Letter-of-Intent 00-002 for PAC 17: {\it Study of the Parity Nonconserving
	Force Between Nucleons Through Deutron Photodisintegration} (2000).

	\bibitem{Woj00} B. Wojtsekhowski and W.~T.~H.~van Oers, {\it Summary of the Working Group Meeting on Parity Violation in Deuteron Photodisintegration with Circularly Polarized Photons}, Jefferson Lab, 13-14 April 2000.
	
	\bibitem{Schindler2010} M. R. Schindler and R. P. Springer, Nucl.\ Phys.\ A {\bf 846}, 51 (2010). 
	
	\bibitem{Vanasse2014} J. Vanasse and M. R. Schindler, Phys. Rev. C {\bf 90}, 044001 (2014).
	
	%crh \bibitem{McDonough1988} J. C. McDonough {\it et al.}, Phys. Rev. D {\bf 38} (1988).
	
	\bibitem{Schindler2013} M. R. Schindler and R. P. Springer, Prog. Part. Nucl. Phys. {\bf 72}, 1 (2013). 
	
	\bibitem{GAS82} J. Gasser and H. Leutwyler, Phys. Rep. C {\bf 87}, 77 (1982).
	\bibitem{GAS84} J.~Gasser and H.~Leutwyler, Ann.\ Phys.\ (N.Y.) {\bf 158}, 142 (1984); Nucl.\ Phys.\ B {\bf 250}, 465 and 539 (1985).

	\bibitem{BKM96B} V. Bernard, N. Kaiser, and Ulf-G. Mei{\ss}ner, {\it Chiral Corrections to the Kroll-Rudermann Theorem}, Bonn University
	preprint TK 96 08, 1996.

	\bibitem{BKM92} V. Bernard {\it et al}., Nucl. Phys. B {\bf 388}, 315 (1992).
	\bibitem{MEI95} Ulf-G. Mei{\ss}ner, private communication, May (1995).

	\bibitem{GIB95} W.~R. Gibbs {\it et al}., Phys. Rev. Lett. {\bf 74} 3740 (1995);  E. Martsinos, preprint ETHZ-IPP, (June 1997).

	\bibitem{BER93} A.~M.~Bernstein, $\pi$N Newsletter {\bf 9} 55 (1993).

	\bibitem{WEI66} S. Weinberg, Phys. Rev. Lett. {\bf 17}, 616 (1966).

	%\bibliography{cgs-sr,ERL-bib,downie,kendellen,miskimen,theory}
	\bibitem{tarawneh-2003} H.~Tarawneh, M. Eriksson, L.-J. Lindgren, B Anderberg,
	%{\it MAX-IV lattice, dynamic properties and magnet system}.
	Nucl. Instrum. Methods A {\bf 508(3)}, 480 (2003).
	
	\bibitem{adriani-2014} O.~Adriani {\it et~al.} EuroGammaS Proposal for the ELI-NP Gamma Beam System (2014).
	
	\bibitem{Alesini-2014} D.~Alesini {\it et~al}, {\it DA$\Phi$NE gamma-rays factory}, 2014.
	
	\bibitem{LRP15} Ani Aprahamian {\it et~al.}, {\it Reaching for the Horizon: The 2015 Long Range Plan for Nuclear Science}, 2015.
	
	\bibitem{Beane:2014ora} S.~R. Beane {\it et~al.},% E.~Chang, S.~Cohen, W.~Detmold, H.~W. Lin, K.~Orginos, A.~Parreno, M.~J. Savage, and B.~C. Tiburzi, 
%{Magnetic moments of light nuclei from lattice quantum chromodynamics}.
	Phys. Rev. Lett. {\bf 113}, 252001 (2014).
	
	\bibitem{Biroth:2015lxa} M.~Biroth, P.~Achenbach, E.~Downie, and A.~Thomas, 
	%{Silicon photomultiplier properties at cryogenic temperatures}.
	Nucl. Instrum. Methods A {\bf 787}, 68 (2015).
	
	\bibitem{Maik} Maik Biroth, personal communication.
	
	\bibitem{Biroth:2016kye} M.~Biroth, P.~Achenbach, E.~Downie, and A.~Thomas.
	%\newblock {Design of the Mainz Active Polarized Target}.
	PoS, PSTP2015:005 (2016).
	
	\bibitem{Chang:2015qxa} E.~Chang {\it et al.}, %W.~Detmold, K.~Orginos, A.~Parreno, M.~J.~Savage, B.~C.~Tiburzi, and S.~R.~Beane.
	%\newblock {Magnetic structure of light nuclei from lattice QCD}.
	Phys. Rev. D {\bf 92}, 114502 (2015).
	
	\bibitem{Zhaoetal} J.-P Chen {\it et~al.},
	{\it Jlab polarized 3He target system}.
	
	\bibitem{Report}
	D.~Drechsel, B.~Pasquini, and M.~Vanderhaeghen,
	%\newblock {Dispersion relations in real and virtual Compton scattering}.
	Phys. Rept. {\bf 378}, 99 (2003).
	
	\bibitem{eriksson-2013} M.~Eriksson {\it et~al},
	%\newblock {Commissioning of the Max IV light source}.
	{\it Proceedings of International Particle Conference, Busan, Korea},
	2016.
	
	\bibitem{dunham-2013} B.~Dunham {\it et~al.},
	%\newblock Record high-average current from a high-brightness photoinjector.
	Appl. Phys. Lett. {\bf 102}, 034105 (2013).
	
	\bibitem{guilliford-2015} C.~Gulliford {\it et~al.},
	%\newblock Demonstration of cathode emittance dominated high bunch charge beams in a dc gun-based photoinjector.
	Appl. Phys. Lett. {\bf 106}, 094101 (2015).
	
	\bibitem{eggl-2016} E.~Eggl {\it et~al.},
	%\newblock The {Munich Compact Light Source}: initial performance measures.
	J. Synchrotron Rad. {\bf 23}, 1137 (2016).
	
	\bibitem{neil-2006} G.R.~Neil {\it et~al.},
	%\newblock The {JLab} high power erl light source.
	Nucl. Instrum. Methods A {\bf 557}, 9 (2006).
	
	\bibitem{Carstens-2014} H.~Carstens {\it et~al.},
	%\newblock Megawatt-scale average-power ultrashort pulses in an enhancement cavity.
	Opt. Lett. {\bf 39}, 2595 (2014).
	
	\bibitem{umemori-2014} K.~Umemori {\it et~al.},
	%\newblock Operation status of {Compact ERL} main linac cryomodule.
	Proc. IPAC 2014, page 2537 (2014).
	
	\bibitem{eichhorn-2016} R.~Eichhorn {\it et~al.},
	%\newblock First cool-down of the cornell {ERL} main linac cryo-module.
	Proc. IPAC 2016, page 2305 (2016).
	
	\bibitem{akagi-2016} T.~Akagi {\it et~al.},
	%\newblock Narrow-band photon beam via laser {Compton} scattering in an energy recovery linac.
	Phys. Rev. Accel. Beams {\bf 19}, 114701 (2016).
	
	\bibitem{farvacque-2013} L.~Farvacque {\it et~al.},
	%\newblock {A low-emittance lattice for the ESRF}.
	{\it Proc. International Particle Conference, Shanghai, China}, 2013.
	
	\bibitem{Freeman:2014kka} W.~Freeman, A.~Alexandru, M.~Lujan, and F.~X.~Lee,
	%\newblock {Sea quark contributions to the electric polarizability of hadrons}.
	Phys. Rev. D {\bf 90}, 054507 (2014).
	
	\bibitem{comptonreview}
	H.~W.~Griesshammer, J.~A.~McGovern, D.~R.~Phillips, and G.~Feldman.
	%\newblock {Using effective field theory to analyse low-energy Compton
	%	scattering data from protons and light nuclei}.
	Prog. Part. Nucl. Phys. {\bf 67}, 841 (2012).
	
	\bibitem{theoryletter}
	H.~W.~Griesshammer, A.~I.~L'vov, J.~A.~McGovern, V.~
	Pascalutsa, B.~Pasquini, and D.~R. Phillips,
	%\newblock {Theory Viewpoint on Extracting Nucleon Polarisabilities in
	%	Low-Energy Compton Scattering}.
	In {\it Compton Scattering off Protons and Light Nuclei Trento, 
			Italy, July 29-August 2, 2013}, 2014.
	
	\bibitem{bernstein-idea} A. Bernstein, private communication.
	
	\bibitem{Kendellen16} D.~P.~Kendellen {\it et~al.}, {\it Nucl. Instrum. Methods A} {\bf 840}, 174 (2016).
	
	\bibitem{Kramer:2007zzb} K.~Kramer {\it et al.}, %X.~Zong, D.~Dutta, H.~Gao, X.~Qian, Q.~Ye, X.~Zhu, R.~Lu, T.~Averett, and S.~Fuchs.
	%\newblock {A high-pressure polarized He-3 gas target for the High Intensity Gamma Source (HIgammaS) facility at Duke Free Electron Laser Laboratory}.
	Nucl. Instrum. Meth. A {\bf 582}, 318 (2007).
	
	\bibitem{Laskaris:2015wma} G.~Laskaris {\it et~al.},
	%\newblock {Measurement of the doubly-polarized $\vec{{^3}He}(\vec{\gamma},n)pp$
	%	reaction at 16.5 MeV and its implications for the GDH sum rule}.
	Phys. Lett. B {\bf 750}, 547 (2015).
	
	\bibitem{Lujan:2016ffj} M.~Lujan, A.~Alexandru, W.~Freeman, and F.~X. Lee,
	%\newblock {Finite volume effects on the electric polarizability of neutral hadrons in lattice QCD}.
	Phys. Rev. D {\bf 94}, 074506 (2016).
	
	\bibitem{Myers:2014ace} L.~S. Myers {\it et~al.},
	%\newblock {Measurement of Compton Scattering from the Deuteron and an Improved Extraction of the Neutron Electromagnetic Polarizabilities}.
	Phys. Rev. Lett. {\bf 113}, 262506 (2014).
	
	\bibitem{Martel15} P.~Martel and the Mainz A2 Collaboration,
	Phys. Rev. Lett. {\bf 114}, 112501 (2015).
	
	\bibitem{Primer:2013pva} T.~Primer, W.~Kamleh, D.~Leinweber, and M.~Burkardt,
	%\newblock {Magnetic properties of the nucleon in a uniform background field}.
	Phys. Rev. D {\bf 89}, 034508 (2014).
	
	\bibitem{Schumacher:2005an} M.~Schumacher,
	%\newblock {Polarizability of the nucleon and Compton scattering}.
	Prog. Part. Nucl. Phys. {\bf 55}, 567 (2005).
	
	\bibitem{Thomas11} A.~Thomas, Eur. Phys. J. Spec. Top. {\bf 198}, 171 (2011).
	
	\bibitem{weller-2009} H.~R. Weller {\it et~al.},
	%\newblock {Research opportunities at the upgraded HI$\gamma$S facility}.
	Prog. Part. Nucl. Phys. {\bf 62}, 257 (2009).
	
	\bibitem{Wright:1985}
	D.~H. Wright, P.~T. Debevec, L.~J. Morford, and A.~M. Nathan,
	%\newblock Elastic photon scattering from carbon and calcium and its
	interpretation.
	Phys.\ Rev.\ C {\bf 32}, 1174 (1985).
	
	\bibitem{ywu-2015} Y.~K.~Wu, ``Light source and accelerator physics research program at Duke University''.
	in {\em Proceedings of International Particle Conference, Richmond, VA,
		USA}, 2015.
	
	\bibitem{Ye:2009dx}
	Q.~Ye {\it et al.}, %G.~Laskaris, H.~Gao, W.~Chen, W.~Zheng, X.~Zong, T.~Averett, G.~D. Cates, and W.~A. Tobias.
	%\newblock {A High-Pressure Polarized He-3 Gas Target for Nuclear Physics
	%	Experiments Using A Polarized Photon Beam}.
	Eur. Phys. J. A {\bf 44}, 55 (2010).
		
	\bibitem{Coo15} N.~Copper, Doctoral Dissertation, Yale University (2015).
	
	\bibitem{Isa16} J.~Isaak, Doctoral Dissertation, Johannes Gutenberg-Universit{\"a}t Mainz (2016).
	
	\bibitem{Isa13} J. Isaak {\it et al.}, Phys. Lett. B {\bf 727}, 361 (2013).
	
	\bibitem{Loh13} B. Loher {\it et al.}, Nucl. Instrum. Methods A {\bf 723}, 136 (2013).
	
	\bibitem{Loh16} B. Loher {\it et al.}, Phys. Lett. B {\bf 756}, 72 (2016).
	
	\bibitem{Pie08} N.~Pietralla, P.~von Brentano, and A.~F.~Lisetskiy, Prog. Part. Nucl. Phys. {\bf 60}, 225 (2008).
	
	\bibitem{Bec17} T. Beck {\it et al.}, Phys. Rev. Lett. {\bf 118}, 212502 (2017).
	
	\bibitem{Bel13} J. Beller {\it et al.}, Phys. Rev. Lett. {\bf 111}, 172501 (2013).
	
	\bibitem{Sav13} D. Savran, T. Aumanna, and A. Zilges, Prog. Part. Nucl. Phys. {\bf 70}, 210 (2013).
	
	\bibitem{Gor98} S. Goriely, Phys. Lett. B {\bf 436}, 10 (1998).
	
	\bibitem{Iac85} F. Iachello, Phys. Lett. B {\bf 160}, 1 (1985).
	
	\bibitem{End10} J. Endres {\it et al.}, Phys. Rev. Lett. {\bf 105}, 212503 (2010).
	
	\bibitem{Kru14} A.~Krugmann, Doctoral Dissertation, Technische Universit{\"a}t Darmstadt (2014).
	
	\bibitem{But96} P. A. Butler and W. Nazarewicz, Rev. Mod. Phys. {\bf 68}, 349 (1996).
	
	\bibitem{Kne06} U. Kneissel, N. Pietralla, and A. Zilges, J. Phys. G {\bf 32}, R217 (2006).
	
	\bibitem{Oer06} W. von Oertzen, M. Freer, and, Y. Kanada-En'yo, Phys. Rep. {\bf 432}, 43 (2006).
	
	\bibitem{Ast10} A. Astier {\it et al.}, Phys. Rev. Lett. {\bf 104}, 042701 (2010).
	
	\bibitem{Roe14} G. Roepke {\it et al.}, Phys. Rev. C {\bf 90}, 034304 (2014).
	
	\bibitem{Pit90} H. H. Pitz {\it et al.}, Nucl. Phys. A {\bf 509}, 587 (1990).
	
	\bibitem{Fri92} H. Friedrichs {\it et al.}, Phys. Rev. C {\bf 45}, R892 (1992).
	
	\bibitem{Eck97} T. Eckert {\it et al.}, Phys. Rev. C {\bf 56}, 1256 (1997).
	
	\bibitem{Spi15} M. Spieker {\it et al.}, Phys. Rev. Lett. {\bf 114}, 192504 (2015).
	
	\bibitem{Eji08} H. Ejiri {\it et al.}, Eur. Phys. J. Special Topics {\bf 162}, 239 (2008).
	
	\bibitem{Ydr12} E. Ydrefors {\it et al.}, Nucl. Phys. A {\bf 896}, 1 (2012).
	
	\bibitem{Pie02} N. Pietralla {\it et al.}, Phys. Rev. Lett. {\bf 88}, 012052 (2002).
	
	\bibitem{Thi02} P. Thirolf and D. Habs, Prog. Part. Nucl. Phys. {\bf 49}, 325 (2002).
	
	\bibitem{Kra11} A. Krasznahorkay, In {\it Handbook of Nuclear Chemistry}, Springer, 2011.
	
	\bibitem{Mcd13} J. McDonnell, W. Nazarewicz, and J. Sheikh, Phys. Rev. C {\bf 87}, 054327 (2013).
	
	\bibitem{Jac13} P. Jachimowicz {\it et al}., Phys. Rev. C {\bf 87}, 044308 (2013).
	
	\bibitem{Csi09} L. Csige {\it et al.}, Phys. Rev. C {\bf 80}, 011301 (2009).
	
	\bibitem{Ber75}  B.~L. Berman and S.~C. Fultz, Rev. Mod. Phys. {\bf 47}, 713 (1975).
	
	\bibitem{Vog01} K. Vogt {\it et al.}, %P. Mohr, M. Babilon, J. Enders, T. Hartmann, C. Hutter, T. Rauscher, S. Volz, A. Zilges, 
	Phys. Rev. C {\bf 63}, 055802  (2001).
	
	\bibitem{Son04} K. Sonnabend, K. Vogt, D. Galaviz, S. M{\"u}ller, and A. Zilges, Phys. Rev. C {\bf 70}, 035802 (2004).
	
	\bibitem{Erh06} M. Erhard {\it et al.}, %A.R. Junghans, R. Beyer, E. Grosse, J. Klug, K. Kosev, C. Nair, N. Nankov, G. Rusev, K.D. Schilling, R. Schwengner, A. Wagner, 
	Eur. Phys. J. A {\bf 27}, s01.135 (2006).
	
	\bibitem{Uts03} H. Utsunomiya {\it et al.}, %H. Akimune, S. Goko, M. Ohta, H. Ueda, T. Yamagata, K. Yamasaki, H. Ohgaki, H. Toyokawa, Y.-W. Lui, T. Hayakawa, T. Shizuma, S. Goriely, 
	Phys. Rev. C {\bf 67}, 015807 (2003).
	
	\bibitem{Sau97} T. Sauter and F. K{\"a}ppeler, Phys. Rev. C {\bf 55}, 3127 (1997).
	
	\bibitem{Bor98} J. Bork, H. Schatz, F. K{\"a}ppeler, and T. Rauscher, Phys. Rev. C {\bf 58}, 524 (1998).
	
	\bibitem{Ozk02} N. {\"O}zkan {\it et al.}, %A.S. J. Murphy, R.N. Boyd, A.L. Cole, M. Famiano, R.T. G{\"u}ray, M. Howard, L. {\c S}ahin, J.J. Zach, R. deHaan, J. G{\"o}rres, M.C. Wiescher, M.S. Islam, T. Rauscher, 
	Nucl. Phys. A {\bf 710}, 469 (2002).
	
	\bibitem{Rap02} W. Rapp {\it et al.}, %M. Heil, D. Hentschel, F. K{\"a}ppeler, R. Reifarth, H.J. Brede, H. Klein, T. Rauscher, 
	Phys. Rev. C {\bf 66}, 015803 (2002).
	
	\bibitem{Gyu05} G. Gy{\"u}rky {\it et al.}, %Z. F{\"u}l{\"o}p, G. Kiss, Z. M{\'a}t{\'e}, E. Somorjai, J. G{\"o}rres, A. Palumbo, M. Wiescher, D. Galaviz, A. Kretschmer, K. Sonnabend, A. Zilges, T. Rauscher, 
	Nucl. Phys. A {\bf 758}, 517 (2005).
	
	\bibitem{Ful01}  Z. F{\"u}l{\"o}p {\it et al.}, %G. Gy{\"u}rky, Z. M{\'a}t{\'e}, E. Somorjai, L. Zolnai, D. Galaviz, M. Babilon, P. Mohr, A. Zilges, T. Rauscher, H. Oberhummer, G. Staudt, 
	Phys. Rev. C {\bf 64}, 065805 (2001).
	
	\bibitem{Gal05} D. Galaviz {\it et al.}, %Z. F{\"u}l{\"o}p, G. Gy{\"u}rky, Z. M{\'a}t{\'e}, P. Mohr, T. Rauscher, E. Somorjai, A. Zilges, 
	Phys. Rev. C {\bf 71}, 065802 (2005).
	
	\bibitem{Kra93}  K.-L. Kratz {\it et al.}, Astrophys. J. {\bf 403}, 216 (1993).
	
	\bibitem{Wall97} G. Wallerstein {\it et al.}, Rev. Mod. Phys. {\bf 69}, 995 (1997).
	
	\bibitem{Abb17} B.P. Abbott {\it et al.} (LIGO and Virgo Collaborations), Phys. Rev. Lett. {\bf 119}, 161101 (2017).
	\bibitem{Kap99} F. K{\"a}ppeler, Prog. Part. Nucl. Phys. {\bf 43}, 419 (1999).
	
	\bibitem{Kap06} F. K{\"a}ppeler and A. Mengoni, Nucl. Phys. A {\bf 777}, 291 (2006).
	
	\bibitem{Dill08}  I. Dillmann, C. Domingo Pardo, F. K{\"a}ppeler, A. Mengoni, and K. Sonnabend, Pub. Astronom. Soc. Australia {\bf 25}, 18 (2008).
	
	\bibitem{Tak83} K. Takahashi and K. Yokoi, Nucl. Phys. A {\bf 404}, 578 (1983).
	
	\bibitem{Bao00} Z.Y. Bao {\it et al.}, At. Data Nucl. Data Tables {\bf 76}, 70 (2000).
	
	\bibitem{Kap11} F. Kappeler {\it et al.}, Rev. Mod. Phys. {\bf 83}, 157 (2011).
	
	\bibitem{Led13} C. Lederer {\it et al.}, Phys. Rev. Lett. {\bf 110}, 022501 (2013).
	
	\bibitem{Led14} C. Lederer {\it et al.}, Phys. Rev. C {\bf 89}, 025810 (2014).
	
	\bibitem{Rau12} T. Rauscher, Astrophys. J. Lett. {\bf 755}, L10 (2012).
	
	\bibitem{Hau52} W. Hauser and H. Feshbach, Phys. Rev. A {\bf87}, 366 (1952).
	
	\bibitem{Ton10} A.P. Tonchev {\it et al.}, Phys. Rev. Lett. {\bf 104}, 072501 (2010).
	
	\bibitem{Loh13} B. Loher {\it et al.}, Nucl. Instrum. Methods A {\bf 723}, 136 (2013).
	
	\bibitem{Rom13} C. Romig {\it et al.}, Phys. Rev. C {\bf 88}, 044331 (2013).
	
	\bibitem{Isa13} J. Isaak {\it et al.}, Phys. Lett. B {\bf 727}, 361 (2013).
	
	\bibitem{Isa16} J. Isaak, Doctoral Dissertation, Universit{\"a}t Mainz (2016), https://publications.ub.uni-mainz.de/theses/volltexte/2016/100000664/pdf/100000664.pdf.
	
	\bibitem{Fow84} W.~A. Fowler, Rev. Mod. Phys. {\bf 56}, 149 (1984).
	
	\bibitem{Str08} F. Strieder, J. Phys. G {\bf 35}, 014009 (2008). 
	
	\bibitem{Sch05} D, Sch{\"u}rmann {\it et al.},  Eur. Phys. J. A {\bf 26}, 301 (2005).
	
	\bibitem{Ass06} M. Assuncao {\it et al.}, Phys. Rev. C {\bf 73} 055801 (2006); M. Fey Doctoral Dissertation, Universit{\"a}t Stuttgart, Germany, 2004.
	
	\bibitem{Mat06} C. Matei {\it et al.}, Phys. Rev. Lett. {\bf 97}, 242503 (2006).
	
	\bibitem{Kun02} R. Kunz {\it et al.}, Astrophys. J. {\bf 567}, 643 (2002).
	
	\bibitem{Gai10} M. Gai {\it et al.}, JINST {\bf 5}, 12004 (2010).
	
	\bibitem{Zim13} W.~R. Zimmerman {\it et al.}, Phys. Rev. Lett. {\bf 110}, 152502 (2013).
	
	\bibitem{DiG15}  B. DiGiovine {\it et al.}, Nucl. Instrum. Methods A {\bf 781}, 96 (2015).
	
	\bibitem{Hae07} P.~Haensel, A.~Y.~Potekhin, and D.~G.~Yakovlev, {\it Neutron Stars 1: Equation of State and Structure} (Springer-Verlag, New York, 2007).
	
	\bibitem{Lat00} J.~M. Lattimer and M. Prakash, Phys. Rep. {\bf 121}, 333 (2000).
	
	\bibitem{Hen11} S.~S. Henshaw {\it et al.}, Phys. Rev. Lett. {\bf 107}, 222501 (2011).
	
	\bibitem{Paa07} N. Paar, D. Vretenar, E. Khan, and G. Colo, Rep. Prog. Phys. {\bf 70}, 691 (2007).
	
	\bibitem{Lit08} E. Litvinova, P. Ring, and V. Tselyaev, Phys. Rev. C {\bf 78}, 014312 (2008).
	
	%\bibitem{Kli07} A. Klimkiewicz {\it et al.}, Phys. Rev. C {\bf 76}, 051603 (2007). {DUPLICATE. Correct form with (R) is six items below]
	
	\bibitem{Pie06} J. Piekarewicz, Phys. Rev. C {\bf 73}, 044325 (2006).
	
	\bibitem{Paa14} N. Paar {\it et al.}, Phys. Rev. C {\bf 90}, 011304(R) (2014).
	
	\bibitem{Kra01} P. G. Krastev and B. A. Li, arXiv:1001.0353. 
	
	\bibitem{Tam11} A. Tamii {\it et al.}, Phys. Rev. Lett. {\bf 107}, 062502 (2011).
	
	\bibitem{Wie09} O. Wieland {\it et al.}, Phys. Rev. Lett. {\bf 102}, 092502 (2009).
	
	\bibitem{Kli07} A. Klimkiewicz {\it et al.}, Phys. Rev. C {\bf 76}, 051603(R) (2007).
	
	
	\bibitem{Pie01a} S.~C. Pieper and V.~R. Pandharipande, Ann. Rev. Nucl. Part. Sci. {\bf 51}, 53  (2001).
	
	\bibitem{Nav07} P. Navratil \emph{et al.}, Phys. Rev. Lett. {\bf 99}, 042501 (2007).
	
	\bibitem{Nav08} P. Navratil \emph{et al.}, Few-Body Syst. {\bf 43}, 129 (2008).
	
	\bibitem{Nog06} A. Nogga, P. Navratil, B.R. Barrett, and J.P. Vary, Phys. Rev. C {\bf 73}, 064002 (2006).
	
	\bibitem{Glo96}  W.  Gl\"ockle \emph{et al.}, Phys. Rep. {\bf 274}, 107 (1996).
	
	\bibitem{Mac01} R. Machleidt, Phys. Rev. C {\bf 63}, 024001 (2001).
	
	\bibitem{Wir95} R.~B.~Wiringa, V.~G.~J.~Stoks, and R.~Schiavilla, Phys. Rev. C {\bf51}, 38 (1995).
	
	\bibitem{Sto94} V.~G.~J.~Stoks, R.~A.~M.~Klomp, C.~P.~F.~Terheggen,  and J.~J.~de Swart, Phys. Rev. C {\bf 49}, 2950 (1994).
	
	\bibitem{Coo75} S.~A. Coon, M.~D. Scadron, and B.~R. Barrett, Nucl. Phys. A {\bf 242}, 467 (1975).
	
	\bibitem{Pie01b} S.~C.~Pieper, V.~R.~Pandharipande, R.~B.~Wiringa, and J.~Carlson, Phys. Rev. C {\bf 64}, 014001 (2001).
	
	\bibitem{Ent03} R. Machleidt and D.R. Entem, Phys. Rep. {\bf 503}, 1 (2011).
	
	\bibitem{Epe09} E.~Epelbaum, H.-W.~Hammer, and Ulf-G.~Meissner, Rev. Mod. Phys. {\bf 81}, 1773 (2009).
	
	\bibitem{Epe11} E.~Epelbaum, H.~Krebs, D.~Lee, and Ulf-G.~Meissner, Phys. Rev. Lett. {\bf 106}, 192501 (2011)
	.
	\bibitem{Bea15} S.~R. Beane {\it et al.}, Phys. Rev. Lett. {\bf 115}, 132001 (2015)
	.
	\bibitem{Gri12} H.~W.~Griesshammer, J.~A.~McGovern, D.~R.~Phillips, and G.~Feldman, Prog. Part. Nucl. Phys. {\bf 67}, 841 (2012).
	
	\bibitem{Bea14} S. Beane \emph{et al.}, Phys. Rev. Lett. \textbf{113}, 252001 (2014).
	
	\bibitem{How16} C.~R.~Howell, W.~Tornow, and H.~Wita{\l}a, EPJ Web of Conferences {\bf 113}, 04008 (2016).
	
	\bibitem{Ber05}  W. Bertozzi and R.J. Ledoux, Nucl. Instrum. Methods B {\bf 241}, 820 (2005).
	
	\bibitem{Pru06} J.~A.~Pruet, D.~P.~McNabb, C.~A.~Hagmann, F.~V.~Hartemann, C.~P.~J.~Barty, J. Appl. Phys. {\bf 99}, 123102 (2006). 
	
	\bibitem{Hag09} C.~A. Hagmann {\it et al.}, J. Appl. Phys. {\bf 106}, 084901 (2009).
	
	%% New references added by CRH on May 21, 2018
	\bibitem{Des80} B.~Desplanques, J.~F.~Donoghue, and B.~R.~Holstein, Ann. Phys. {\bf 124}, 449 (1980).
	
	\bibitem{Sch04} R. Schiavilla, J. Carlson, and M. Paris, Phys. Rev. C {\bf 70}, 044007 (2004).
	
	\bibitem{Bow07} J. Bowman, INT program "Fundamental Neutron Physics" (2007), http://www.int.washington.edu/talks/WorkShops/int\_07\_1/.
	
	%\bibitem{Sav99} M.J. Savage, K.A. Scaldeferri, and M.B. Wise, Nucl. Phys. A {\bf 652}, 273 (1999).
\bibitem{Ots05}  T. Otsuka and others, Phys. Rev. Letts. {\bf 95}, 232502 (2005).
\bibitem{Ots16}  T. Otsuka and Y. Tsunoda, J. Phys. G: Nucl. Part. Phys. {\bf 43}, 024009 (2016).
\bibitem{Leo17}  S. Leoni and others, Phys. Rev. Letts. {\bf 118}, 162502 (2017), B. P. Crider, \it{et al.}, Phys. Letts. B {\bf 763}, 108 (2016), S. Suchyta \it{et al.}, Phys. Rev. C {\bf 89}, 021301(R) (2014)
\end{thebibliography}

%REFERENCES BELOW ARE ALL DUPLICATES. There is one that CRH commented out (his initials) both below and early in the list.

	%\bibitem{Bec01} D. H. Beck and B. Holstein, Int. J. Mod. Phys. E {\bf 10}, 1 (2001). [DUPLICATE]
	
	%\bibitem{Beck01} D. H. Beck and R. D. McKeown, Ann. Rev. Nucl. Part. Sci. {\bf 51}, 189 (2001). [DUPLICATE]
	
	%\bibitem{Beck03} D. H. Beck, Prog. Nucl. Part. Phys. {\bf 50}, 429 (2003). [DUPLICATE]
	
	%\bibitem{Beise05} E. J. Beise, M. L. Pitt, and D. T. Spayde, Prog. Nucl. Part. Phys. {\bf 54}, 289 (2005). [DUPLICATE]
	
	%\bibitem{Ade85} E.~G.~Adelberger and W.~C.~Haxton, Ann. Rev. Nucl. Part. Sci. {\bf 35}, 501 (1985). [DUPLICATE]
	
	%\bibitem{Bow1} J.~D.~Bowman, G.~T.~Garvey, and M.~B.~Johnson, Ann. Rev. 
	Nucl. Part. Sci. {\bf 43}, 829 (1993). [DUPLICATE]
	
	%\bibitem{Tom} S.~Tomsovic, M.~B.~Johnson, A.~Hayes, and J.~D.~Bowman, 
	Phys. Rev. C {\bf 62}, 054607 (2000). [DUPLICATE]
	
	%\bibitem{Woo97} C.~S. Wood et al., Science {\bf 275}, 1759 (1997). [DUPLICATE]
	
	%\bibitem{Zel57} Y. B. Zeldovich, Sov. Phys. JETP {\bf 6}, 1184 (1957). [DUPLICATE]
	
	%\bibitem{Fla80} V. V. Flambaum and I. B. Khriplovich, Sov. Phys. JETP {\bf 52}, 835 (1980). [DUPLICATE]
	
	%\bibitem{Tsi09}K. Tsigutkin {\it et al.}, Phys. Rev. Lett. {\bf 103}, 071601 (2009). [DUPLICATE]
	
	%\bibitem{Pre03} G. Prezeau, M. Ramsey-Musolf, and P. Vogel, Phys. Rev. D {\bf 68}, 034016 (2003). [DUPLICATE]
	
	%\bibitem{Bowman2014} J. D. Bowman and V. Gudkov, Phys. Rev. C {\bf 90}, 065503 (2014). [DUPLICATE]
	
	%\bibitem{Wasem12} J. Wasem, Phys. Rev. C {\bf 85}, 022501(R) (2012). [DUPLICATE]
	
	%\bibitem{KITP} Frontiers in Nuclear Physics, KITP workshop,  Aug. 22-Nov. 4, 2016. [DUPLICATE]
	
	%\bibitem{Dan} G. S. Danilov, Phys. Lett. {\bf 18}, 40 (1965). [DUPLICATE]
	%\bibitem{Zhu05} S. L. Zhu {\it et al.}, Nucl. Phys. A {\bf 748}, 435 (2005). [DUPLICATE]
	%\cite{Girlanda:2008ts}
	%\bibitem{Girlanda:2008ts} L.~Girlanda,
	%``On a redundancy in the parity-violating 2-nucleon contact Lagrangian,''
	%Phys.\ Rev.\ C {\bf 77}, 067001 (2008) 	[arXiv:0804.0772 [nucl-th]]. [DUPLICATE]
	%%CITATION = ARXIV:0804.0772;%%
	
	
	%\bibitem{Phillips:2014kna} D.~R.~Phillips, D.~Samart, and C.~Schat, 	Phys.\ Rev.\ Lett.\  {\bf 114}, 062301 (2015). [DUPLICATE]
	
	%\bibitem{Schindler2016} M. R. Schindler, R. P. Springer, and J. Vanasse, Phys. Rev. C {\bf 93}, 025502 (2016). [DUPLICATE]
	
	%\bibitem{Snow2015} W. M. Snow {\it et al.}, Rev. Sci. Instrum. {\bf 86}, 055101 (2015). [DUPLICATE]
	
	%\bibitem{INCITE} A.~Walker-Loud, E. Berkowitz, W. Haxton, T. Kurth,  A. Nicholson, and J. Wasem, 2016 Incite Award, First Lattice QCD Calculation of the I=2 Two-Nucleon Parity Violating Amplitude. [DUPLICATE]
	***
	%\bibitem{Kurth:2015cvl} T.~Kurth {\it et al.}, %E.~Berkowitz, E.~Rinaldi, P.~Vranas, A.~Nicholson, M.~Strother, A.~Walker-Loud and E.~Rinaldi,
	%``Nuclear Parity Violation from Lattice QCD,''
	%PoS LATTICE {\bf 2015}, 329 (2016). [DUPLICATE]
	
	%\bibitem{Earle88} E. D. Earle {\it et al.}, %A. B. McDonald, S. H. Kinder, E. T. H. Clifford, J. J. Hill, G. H. Keech, T. E. Chupp, and M. B. Schneider, Canadian Journal of Physics {\bf 66}, 534 (1988). [DUPLICATE]
	
	%\cite{Knyaz'kov:1984zz}
	%\bibitem{Knyaz'kov:1984zz} V.~A.~Knyaz'kov {\it et al.}, %E.~A.~Kolomenskii, V.~M.~Lobashov, V.~A.~Nazarenko, A.~N.~Pirozhkov, A.~I.~Shablii, E.~V.~Shul'gina and Y.~V.~Sobolev,
	%``A new experimental study of the circular polarization of np capture gamma-rays,''
	%Nucl.\ Phys.\ A {\bf 417}, 209 (1984). [DUPLICATE]
	%%CITATION = NUPHA,A417,209;%%
	
	%\bibitem{Sinclair00} C. Sinclair  {\it et al.}, Letter-of-Intent 00-002 for PAC 17: {\it Study of the Parity Nonconserving Force Between Nucleons Through Deutron Photodisintegration}, (2000). [DUPLICATE]
	%\bibitem{Woj00} B.~Wojtsekhowski and W.~T.~H.~van Oers, {\it Summary of the Working Group Meeting on Parity Violation in Deuteron Photodisintegration with Circularly Polarized Photons}, Jefferson Lab, 13-14 April 2000. [DUPLICATE]
	
	%\bibitem{Schindler2010} M. R. Schindler and R. P. Springer, Nucl.\ Phys.\ A {\bf 846}, 51 (2010). [DUPLICATE of a much earlier entry]
	
	%\bibitem{Vanasse2014} J. Vanasse, M. R. Schindler, Phys. Rev. C {\bf 90}, 044001 (2014). [DUPLICATE]
	
	%crh \bibitem{McDonough1988} J. C. McDonough {\it et al.}, Phys. Rev. D, {\bf 38} (1988).
	
	%\bibitem{Schindler2013} M. R. Schindler, R. P. Springer, Prog. Part. Nucl. Phys.  (2013). [DUPLICATE]


